Toward Optimal Run Racing: Application to Deep Learning Calibration

This paper aims at one-shot learning of deep neural nets, where a highly parallel setting is considered to address the algorithm calibration problem - selecting the best neural architecture and learning hyper-parameter values depending on the dataset at hand. The notoriously expensive calibration problem is optimally reduced by detecting and early stopping non-optimal runs. The theoretical contribution regards the optimality guarantees within the multiple hypothesis testing framework. Experimentations on the Cifar10, PTB and Wiki benchmarks demonstrate the relevance of the approach with a principled and consistent improvement on the state of the art with no extra hyper-parameter.

==> Conc_old.tex <==
{\bf{Validation of the method in \cite{Domhan}.}} Results vary in terms of impact, but we confirm the stability of the method proposed in \cite{Domhan}, sometimes saving up more than 85\%. The impact was greater for images than for language modelling. We can apply it both at the level of multiple runs with randomized hyperparameters, and at the level of different models - each of them usually based on randomized hyperparameters. Cumulating both levels can decrease the computational cost by more than a factor 10 as shown by our Cifar and Metacifar experiments.
{\bf{The threshold $\delta$ (0.05 in \cite{Domhan})}} is probably not very important; we get stable results even with 0.5, because the regression is, by the nature of models and in the settings we consider, conservative.
{\bf{The performance is only marginally better than the original method at least when the original method was tuned}}. Clever-halt(f) is nonetheless more principled, and excellent independently of $\delta$, and if the improvement is moderate, it is perfectly stable (Fig.\ref{compa} and supplementary material). 
{\bf{Novelty:}} Adding predictions into the halting threshold is new, and the idea of using a quantile of the predictions rather than the best prediction, in an adaptive manner, is new and robust; this principle (applied to job pruning), maybe rather than the exact derivation of risks, is the key conclusion of this paper.
%Further work = ensemble methods; with e.g. clearing methods we might get ensembles at a moderate cost.


==> Intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The algorithm selection problem $-$ aimed at selecting {\em a priori} the learning algorithm  best suited to a given dataset $-$ and the algorithm calibration problem $-$ aimed at identifying the best hyper-parameter setting of an algorithm for this dataset $-$ have been acknowledged a key issue since the late 80s  \cite{Bradzil00,Bardenet11,thornton2013AutoWeka,Bardenet13,Pfahringer13,Kalousis14}.
Several challenges have been organized to further investigate both algorithm selection and calibration issues in the last few years \cite{AutoML16-ICML,AutoML15-NIPS}. 
\def\DNN{{DNN}}

The algorithm selection issue appears settled as of now, at least in the case where sufficient training data is available: deep learning (\DNN) consistently delivers dominant performances in many application domains, and is currently considered to the best learning algorithm in the large data regime  \cite{cifar10,Donahue,Deng,Atari,AlphaGo}.
This renders the algorithm calibration an even more critical issue: on the one hand, \DNN\ training notoriously requires high computational resources; on the other hand, it involves a structured hyper-parameter space, hindering the approximation of the performance model (more in section \ref{sec:soa}). 
Automatic algorithm calibration thus is challenged by {manual} algorithm calibration, as noted by \cite{Domhan}. As the experienced practitioner can easily detect and stop the unpromising runs based on their learning curves in the first epochs, she can afford to consider many more hyper-parameter settings. 

How to discard as early as possible runs/solutions that will eventually yield under-optimal results has long and thoroughly been investigated in the literature in a variety of contexts (see for instance \cite{Igel-ICML09,Domhan}; section \ref{sec:soa}). The early discard decision problem raises two interdependent questions: uncertainty modelling, as the eventual quality of a run result is unknown until the run is achieved; the guarantees to be provided about the overall process, typically the risk of stopping and discarding a run which would have yielded the best result.

This paper addresses the early discard problem in the context of parallel one-shot deep neural training. Formally, the considered framework, referred to as  parallel one-shot run race (\PORR), allocates all available computational resources at the beginning of the period to train deep neural nets; each core runs with its specific hyper-parameter setting), all starting at the beginning of the period. 
\def\PORR{PaRR}
The problem is a constrained optimization problem: i) the constraint regards the  optimality guarantee to be provided about ensuring that the best run lives until the end of the period; ii) the optimization consists of minimizing the computational budget subject to the optimality guarantee, by stopping any run (with no possible resuming of the run, as opposed to \cite{freezethaw}) as early as possible.  

The \PORR\ decision maker aims at rendering Deep Learning robust w.r.t. random hazards (e.g. initializations) and bad decisions (e.g. hyper-parameter setting set), delivering at the end of the period the optimal model out of the predefined hyper-parameter setting set,  with a minimal computational budget (noting that the computational budget is upper bounded by the number of GPUs and the length of the training period by construction). The challenge lies in making the stopping decision with little and censored evidence: as all runs are simultaneous, only prior information about the learning curves behavior is available, as in \cite{Domhan}, and by construction the system does not have any information about what would have been the behavior of runs after they are stopped. 

%an optimality guarantee with a lower overall computational cost than 
%provided using e.g. ensemble methods \cite{hyperband},
Compared to e.g. Hyperband\cite{hyperband}, curve modeling as in \cite{domhan} provides important advantages: whereas Hyperband uses several independent sequential halving, we can prune arbitrarily many curves based on a few single runs;
and we can adapt this method to any deep learning platform, whereas Hyperband requests a rate $\eta$ at which we discard runs - so that the number of discarded runs can not depend on the shape of curves, a dangerous situation in the common case in which validation curves are very noisy at the beginning or when one of the parameters (typically the time step at which we start learning rate decay) has a late impact so that all curves are approximately the same at the beginning.
The contribution of the paper is to independently reproduce the method in \cite{domhan} and to provide a principled method improving it without adding any parameter,
 through (i) the use of prediction in the choice of thresholds used for stopping some runs and (ii) a consistent treatment of the multiple hypothesis testing issue. The experimentations on the Cifar, PTB, MiniWiki benchmarks show a consistent improvement compared to the state of the art\cite{Domhan}, for each and every value of the parameter $\delta$. This paper is organized as follows. Section \ref{sec:soa} briefly discusses related work. Section \ref{sec:algo} describes several levels of guarantees and the associated decision criteria, which will be empirically compared and assessed in section \ref{sec:expe}.




==> Intro_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The algorithm selection problem $-$ aimed at selecting {\em a priori} the learning algorithm  best suited to a given dataset $-$ and the algorithm calibration problem $-$ aimed at identifying the best hyper-parameter setting of an algorithm for this dataset $-$ have been acknowledged a key issue since the late 80s  \cite{Bradzil00,Bardenet11,thornton2013AutoWeka,Bardenet13,Pfahringer13,Kalousis14}.
Several challenges have been organized to further investigate both algorithm selection and calibration issues in the last few years \cite{AutoML16-ICML,AutoML15-NIPS}. 
\def\DNN{{DNN}}

The algorithm selection issue appears settled as of now, at least in the case where sufficient training data is available: deep learning (\DNN) consistently delivers dominant performances in many application domains, and is currently considered to the best learning algorithm in the large data regime  \cite{KrizhevskySH12,Donahue,Deng,Atari,AlphaGo}.
This renders the algorithm calibration an even more critical issue: on the one hand, \DNN\ training notoriously requires high computational resources; on the other hand, it involves a structured hyper-parameter space, hindering the approximation of the performance model (more in section \ref{sec:soa}). 
Automatic algorithm calibration thus is challenged by {manual} algorithm calibration, as noted by \cite{Domhan}. As the experienced practitioner can easily detect and stop the unpromising runs based on their learning curves in the first epochs, she can afford to consider many more hyper-parameter settings. 

How to discard as early as possible runs/solutions that will eventually yield under-optimal results has long and thoroughly been investigated in the literature
inin a variety of contexts (see for instance \cite{Igel-ICML09,Domhan}; section \ref{sec:soa}). The early discard decision problem raises two interdependent questions: uncertainty modelling, as the eventual quality of a run result is unknown until the run is achieved; the guarantees to be provided about the overall process, typically the risk of stopping and discarding a run which would have yielded the best result.

This paper addresses the early discard problem in the context of parallel one-shot deep neural training. Formally, the considered framework, referred to as  parallel one-shot run race (\PORR), allocates all available computational resources at the beginning of the period to train deep neural nets; each core runs with its specific hyper-parameter setting with no communication among the cores.

The \PORR\ problem is a constrained optimization problem: i) the constraint regards the  optimality guarantee to be provided about eventually delivering the optimal results, i.e. ensuring that the best run lives until the end of the period; ii) the optimization consists of minimizing the computational budget subject to the optimality guarantee, by stopping any run (with no possible resuming of the run, as opposed to \cite{freezethaw}) as early as possible.  

The \PORR\ decision maker aims at rendering Deep Learning robust w.r.t. random hazards (e.g. initializations) and bad decisions (e.g. hyper-parameter setting set), delivering at the end of the period the optimal model out of the predefined hyper-parameter setting set,  with a minimal computational budget.
%(noting that the computational budget is upper bounded by the number of GPUs and the length of the training period by construction). 
The challenge lies in making the stopping decision with little and censored evidence: as all runs are simultaneous, only prior information about the learning curves behavior is available, as in \cite{Domhan}, and by construction the system does not have any information about what would have been the behavior of runs after they are stopped. 

%an optimality guarantee with a lower overall computational cost than 
%provided using e.g. ensemble methods \cite{hyperband},
The present paper, building upon the current best approach \cite{domhan}, makes theoretical and empirical contributions. On the theoretical side and with no additional hyper-parameter, a principled approach is used to set the discarding thresholds; furthermore, guarantees are obtained through a consistent treatment of the multiple hypothesis testing issue. On the empirical side, the experimentations on the Cifar \cite{cifar}, PTB, and MiniWiki benchmarks show a consistent improvement compared to  \cite{Domhan}, for each and every hyper-parameter setting.

 This paper is organized as follows. Section \ref{sec:soa} briefly discusses related work. Section \ref{sec:algo} describes several levels of guarantees and the associated decision criteria, which will be empirically compared and assessed in section \ref{sec:expe}.




==> Related.tex <==
\section{Related work}\label{sec:soa}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The algorithm selection and calibration issues have been extensively considered in many domains related to combinatorial optimization, ranging from propositional satisfiability and constraint satisfaction to  machine learning and data mining.

Running many learnings simultaneously makes machine learning robust to unlucky initializations and to bad hyperparameter choice, and permits ensemble methods\cite{ensemblehp}. This is however an expensive task; a recent trend in the literature is to ``kill' useless runs when it becomes obvious that the results will not be very good. This is close to what humans would do, i.e. watch validation curves during the training and stop the worst learnings.
The bandit literature is a nature candidate for pruning multiruns. Sequential halving ``kills'' at some predefined time steps half currently running algorithms \cite{seqhal}.
\cite{hyperband} uses several independent instances of sequential halving for making it robust to parameter choice. \cite{domhan} uses Bayesian inference for modelling the validation curves and uses the resulting confidence intervals for deciding which curves should be killed.
We consider the fully parallel setting; maybe our approach could be combined with iterative methods like Gaussian Processes\cite{gpmlTODO}, or variants without stochastic modeling\cite{hord}; and/or with methods such as \cite{freezethaw} which uses stop/resume. The point of the present paper is to focus on (i) the fully parallel setting (ii) constraint that killing the best run is very unlikely (iii) goal = minimization of the overall computational cost (within constraint (ii) ). 

\subsection{Difference with the state of the art}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our setting is different from the one considered in various existing papers.
Hyperband uses independent sequential halvings, making a strong pruning unlikely whenever one run would outperform all others by far; it also does not use the shape of curves - if $N$ validation curves are indistinguishable we might nonetheless kill half of them just because we reach the time step at which half curves should be killed; therefore requirement (ii) can not be fullfilled.
We heavily use the methods in \cite{domhan}; the key difference is the fully parallel setting, which makes the killing criterion in \cite{domhan} not good enough. In particular the method in \cite{domhan} will not kill any of $N$ runs, even if they are perfectly similar except a constant gap in favor of one of them and if there is a perfect fit with negligible confidence intervals - \cite{domhan} uses the current best validation as a threshold, which is not enough in such a setting. 

blabla
% Maybe to be cited: http://akshayc.com/publications/ecml2017_gelc_submitted.pdf (using previous builds)


